Grounding DINO: Marrying DINO with Grounded Pre-Training for Open-Set Object Detection

In this paper, we present an open-set object detector, called Grounding DINO, by marrying Transformer-based detector DINO with grounded pre-training, which can detect arbitrary objects with human inputs such as category names or referring expressions. The key solution of open-set object detection is introducing language to a closed-set detector for open-set concept generalization. To effectively fuse language and vision modalities, we conceptually divide a closed-set detector into three phases and propose a tight fusion solution, which includes a feature enhancer, a language-guided query selection, and a cross-modality decoder for cross-modality fusion. While previous works mainly evaluate open-set object detection on novel categories, we propose to also perform evaluations on referring expression comprehension for objects specified with attributes. Grounding DINO performs remarkably well on all three settings, including benchmarks on COCO, LVIS, ODinW, and RefCOCO/+/g. Grounding DINO achieves a $52.5$ AP on the COCO detection zero-shot transfer benchmark, i.e., without any training data from COCO. It sets a new record on the ODinW zero-shot benchmark with a mean $26.1$ AP. Code will be available at \url{https://github.com/IDEA-Research/GroundingDINO}.

==> image_tex/hero_image.tex <==
\begin{figure*}[!htbp]
    \centering
    \includegraphics[width=0.9\linewidth]{resources/hero_image.pdf}
    \caption{
    (a) A good open-world object detector should work well in all three settings: close-set object detection, open-set object detection, and visual grounding. We hope it is a more comprehensive evaluation of open-world object detectors. (b) We provide an image editing application by combining Grounding DINO and stable diffusion \cite{rombach2021highresolution}.
    }
    \label{fig:hero_image}
\end{figure*}

==> image_tex/task_relation.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.96\linewidth]{resources/task_relation.pdf}
    \vspace{-0.3cm}
    \caption{
    A good open-world object detector should work well on all the three settings: close-set object detection, open-set object detection, and visual grounding. We hope it is a more comprehensive evaluation for open-world object detectors.
    % We view close-set object detection, open-set object detection, and visual grounding as three sub-tasks of open-world object detection. 
    }
    \label{fig:task_relation}
    % \vspace{-0.8cm}
\end{figure}

==> sec/02_introduction.tex <==
\section{Introduction}
\label{sec:intro}


% task def & importance
Understanding novel concepts is a fundamental capability of visual intelligence. In this work, we aim to develop a strong system to detect arbitrary objects specified by human language inputs, which we name as \textit{open-set object detection}\footnote{We view the terms \textit{open-set object detection}, \textit{open-world object detection}, and \textit{open-vocabulary object detection} the same task in this paper. To avoid confusion, we always use \textit{open-set object detection} in our paper.}. The task has wide applications for its great potential as a generic object detector. For example, we can cooperate it with generative models for image editing (as shown in Fig. \ref{fig:hero_image} (b)). 



The key to open-set detection is introducing language for unseen object generalization \cite{li2021grounded, peterAnderson2017BottomUpAT, JiajunDeng2021TransVGEV}. For example, GLIP \cite{li2021grounded} reformulates object detection as a phrase grounding task and introduces contrastive training between object regions and language phrases. It shows a great flexibility for heterogeneous datasets and remarkable performance on both closed-set and open-set detection. Despite its impressive results, GLIP's performance can be constrained since it is designed based on a traditional one-stage detector Dynamic Head \cite{dai2021dynamic}. As open-set and closed-set detection are closely related, we believe a stronger closed-set object detector can result in an even better open-set detector. 

Motivated by the encouraging progress of Transformer-based detectors \cite{zhang2022dino, liu2022dabdetr, li2022dn, FengLi2023MaskDT}, in this work, we propose to build a strong open-set detector based on DINO \cite{zhang2022dino}, which not only offers the state-of-the-art object detection performance, but also allows us to integrate multi-level text information into its algorithm by grounded pre-training. We name the model as \textbf{Grounding DINO}. 
Grounding DINO has several advantages over GLIP. First, its Transformer-based architecture is similar to language models, making it easier to process both image and language data. For example, as all the image and language branches are built with Transformers, we can easily fuse cross-modality features in its whole pipeline. Second, Transformer-based detectors have demonstrated a superior capability of leveraging large-scale datasets. Lastly, as a DETR-like model, DINO can be optimized end-to-end without using any {hand-crafted} modules such as NMS (Non-Maximum Suppression), which greatly simplifies the overall grounding model. 

\input{image_tex/model_comparison}


Most existing open-set detectors are developed by extending closed-set detectors to open-set scenarios with language information. As shown in Fig.  \ref{fig:model_comparison}, a closed-set detector typically has three important modules, a backbone for feature extraction, a neck for feature enhancement, and a head for region refinement (or box prediction). A closed-set detector can be generalized to detect novel objects by learning language-aware region embeddings so that each region can be classified into novel categories in a language-aware semantic space. The key to achieving this goal is using contrastive loss between region outputs and language features at the neck and/or head outputs.  
To help a model align cross-modality information, some work tried to fuse features before the final loss stage. Fig.  \ref{fig:model_comparison} shows that feature fusion can be performed in three phases: neck (phase A), query initialization (phase B), and head (phase C). For example, GLIP \cite{li2021grounded} performs early fusion in the neck module (phase A), and OV-DETR \cite{YuhangZang2022OpenVocabularyDW} uses language-aware queries as head inputs (phase B). 

We argue that more feature fusion in the pipeline enables the model to perform better. 
It is worth noting that retrieval tasks prefer a CLIP-like two-tower architecture which only performs multi-modality feature comparison at the end for efficiency. However, for open-set detection, the model is normally given both an image and a text input that specifies the target object categories or a specific object. In such a case, a tight (and early) fusion model is more preferred for a better performance \cite{peterAnderson2017BottomUpAT, li2021grounded} as both image and text are available at beginning. 
Although conceptually simple, it is hard for previous work to perform feature fusion in all three phases. The design of classical detectors like Faster RCNN makes it hard to interact with language information in most blocks. Unlike classical detectors, the Transformer-based detector DINO has a consistent structure with language blocks. The layer-by-layer design enables it to interact with language information easily. 
Under this principle, we design three feature fusion approaches in the neck, query initialization, and head phases. More specifically, we design a feature enhancer by stacking self-attention, text-to-image cross-attention, and image-to-text cross-attention as the neck module. We then develop a language-guided query selection method to initialize queries for head. We also design a cross-modality decoder for the head phase with image and text cross-attention layers to boost query representations. The three fusion phases effectively help the model achieve better performance on existing benchmarks, which will be shown in Sec. \ref{sec:ablations}. 


% the pity in previous work -> or def of owod
Although significant improvements have been achieved in multi-modal learning, most existing open-set detection work evaluates their models on objects of novel categories, as shown in the left column of Fig.  \ref{fig:hero_image} (b). We argue that another important scenario, where objects are described with attributes, should also be considered. 
In the literature, the task is named Referring Expression Comprehension (REC) \cite{Miao2022ReferringEC, JingyuLiu2017ReferringEG}\footnote{We use the term \textit{Referring Expression Comprehension (REC)} and \textit{Referring (Object) Detection} exchangeable in this paper.}. We present some examples of REC in the right column of Fig.  \ref{fig:hero_image} (b). It is a closely related field but tends to be overlooked in previous open-set detection work.
In this work, we extend open-set detection to support REC and also evaluate its performance on REC datasets.


We conduct experiments on all three settings, including closed-set detection, open-set detection, and referring object detection, to comprehensively evaluate open-set detection performance. 
Grounding DINO outperforms competitors by a large margin. For example, Grounding DINO reaches a $52.5$ AP on COCO minival without any COCO training data. It also establishes a new state of the art on the ODinW \cite{ChunyuanLi2022ELEVATERAB} zero-shot benchmark with a $26.1$ mean AP. 




% The contributions of this paper are summarized as follows:
% \begin{enumerate}[itemsep=0pt, topsep=0pt, parsep=0pt]
% \item We propose Grounding DINO, which extends a closed-set detector DINO by performing vision-language modality fusion at multiple phases, including a feature enhancer, a language-guided query selection module, and a cross-modality decoder. Such a deep fusion strategy effectively improves open-set object detection.
% \item We propose to extend the evaluation of open-set object detection to REC datasets. It helps evaluate the performance of the model with freeform text inputs.
% \item The experiments on COCO, LVIS, ODinW, and RefCOCO/+/g datasets demonstrate the effectiveness of Grounding DINO on open-set object detection tasks.
% \end{enumerate}

\input{tables/related_work4.tex}

==> sec/reproducibility.tex <==
\paragraph{Reproducibility}

We will make our code open-source, as well as our online demo. Additionally, we will elucidate our model training parameters, implementation details, and details of training data within this paper, as shown in Sec. \ref{sec:exp}, Sec. \ref{sec:imple_details}, and Sec. \ref{sec:data_usage}, to ensure transparency and reproducibility of our model.

==> tables/LVIS_finetune.tex <==
% \begin{table}[!htbp]
\begin{wraptable}{r}{0.5\linewidth}


% \begin{center}
% \small
\resizebox{\linewidth}{!}{
\begin{tabular}{l@{\hskip9pt} l@{\hskip9pt} |
c@{\hskip9pt} | c@{\hskip9pt}c@{\hskip9pt} }
% c@{\hskip9pt} c@{\hskip9pt}}
\toprule

\multirow{2}{*}{Model} & 
\multirow{2}{*}{Backbone} &
\multirow{2}{*}{Pre-Training Data} &
\multicolumn{2}{c}{MiniVal \cite{kamath2021mdetr}} \\
 && & AP & APr/APc/APf  \\
\midrule
 GLIPv2* \cite{zhang2022glipv2} &  Swin-T & O365,GoldG,Cap4M & 50.6 &  - / - / -    \\
DetCLIPv2 \cite{yao2023detclipv2} & Swin-T & O365,GoldG,CC15M  & 50.7 & 44.3/52.4/{50.3}    \\
\midrule
\rowcolor{Gray} Grounding DINO T  & Swin-T & O365,GoldG  & \textbf{52.1} & 35.4/51.3/55.7 \\
\bottomrule
\end{tabular}


}
\caption{Fine-tuning performance on LVIS. *The models are trained with mask annotation. }
\label{table:lvis_finetune}
% \end{center}
% \vspace{-6mm}
\end{wraptable}

==> tables/comparison.tex <==
\begin{table*}[t]
\caption{Model Comparisons. }
\label{table:cocomain}
\begin{center}
\resizebox{0.9\linewidth}{!}{
\begin{tabu}{l@{\hskip9pt} 
c@{\hskip9pt} | c | c 
c  c@{\hskip9pt}c@{\hskip9pt}
 }
\toprule
\multirow{2}{*}{Model} & 
\multicolumn{}{}{Backbone} & 
\multirow{2}{*}{Backbone} & 
\multirow{2}{*}{Pre-Train Data}  &
{Zero-Shot}  & Fine-Tune   \\
 & 
 & 
 &
\small{2017val}  & \small{2017val }   \\
\midrule
\rowfont{\color{darkgray}}
Faster R-CNN & RN50-FPN & -  & - & 40.2 / - \\
\rowfont{\color{darkgray}}
Faster R-CNN & RN101-FPN & -  & - & 42.0 / - \\
\rowfont{\color{darkgray}}
DyHead-T \cite{dai2021dynamic} & Swin-T & - & - & 49.7 / - \\
\rowfont{\color{darkgray}}
DyHead-L \cite{dai2021dynamic} & Swin-L & - & - & 58.4 / 58.7 \\
\rowfont{\color{darkgray}}
DyHead-L \cite{dai2021dynamic} & Swin-L  & O365,ImageNet21K  & - & 60.3 / 60.6\\
\rowfont{\color{darkgray}} SoftTeacher \cite{xu2021end} & Swin-L  & O365,SS-COCO & - & 60.7 / 61.3 \\
\rowfont{\color{darkgray}} DINO(Swin-L) \cite{zhang2022dino} & Swin-L  & O365 & - & 62.6 / 62.6 \\
\midrule

DyHead-T & Swin-T &  O365   & 43.6 & 53.3 / - \\
GLIP-T (B)  & Swin-T     & O365  & 44.9 & 53.8 / - \\
GLIP-T (C)  & Swin-T     & O365,GoldG & {46.7} & 55.1 / - \\
GLIP-L  & Swin-L  & FourODs,GoldG,Cap24M & {49.8} & {60.8} / 61.0 \\
\midrule
DINO(Swin-T) \cite{zhang2022dino} & Swin-T & O365 & 46.2  & 56.9 / - \\
Grounding DINO T   & Swin-T    & O365    & 46.7  & 56.9 / -  \\
Grounding DINO T   & Swin-T    & O365,GoldG    & 48.1  & 57.1 / -  \\
Grounding DINO L   & Swin-L    & O365,OI,GoldG,PhCut    & 52.5  & 62.6 / (\shilong{TODO})  \\
   &     &     &   &  63.0 / (\shilong{TODO})  \\
\bottomrule
\end{tabu}
}
\end{center}
\vspace{-4mm}
\end{table*}

==> tables/related_work.tex <==
\begin{table*}[h]
\begin{center}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabu}{
l@{\hskip9pt} |  
c@{\hskip9pt} c@{\hskip9pt}  c@{\hskip9pt} |
c@{\hskip9pt} |
c@{\hskip9pt} |
c@{\hskip9pt} c@{\hskip9pt}  c@{\hskip9pt}  c@{\hskip9pt} |
c@{\hskip9pt} c@{\hskip9pt}  c@{\hskip9pt}  }
 \toprule
 \multirow{2}{*}{Model}  & 
 \multicolumn{3}{c|}{Model Design}  & 
 \multicolumn{1}{c|}{Text Prompt}  & 
 \multicolumn{1}{c|}{Close-Set Settings} &
 \multicolumn{4}{c|}{Open-Set Settings} & 
 \multicolumn{3}{c}{Visual-Grounding Settings}  \\
  & 
  Base Detector & Fusion Phases (Fig. \ref{fig:model_comparison}) & CLIP-dependent & 
  Representation Level & 
  COCO & 
  LVIS zero-shot & ODinW zero-shot & ODinW few-shot & ODinW full-shot &
  PEG & Phrase Grounding & REC \\
\midrule
  ViLD \cite{XiuyeGu2021OpenvocabularyOD} & Mask R-CNN \cite{he2017mask} & 3,4 & \checkmark & sentence & & \checkmark &&& &&& \\
  RegionCLIP \cite{YiwuZhong2022RegionCLIPRL} & Faster RCNN \cite{faster-rcnn} & 4 & \checkmark & sentence & \checkmark & \checkmark & & & & & & \\
  FindIt \cite{WeichengKuo2022FindItGL} & Faster RCNN \cite{faster-rcnn} & 3,4 &  & sentence & \checkmark & & & & & & & \checkmark \\
  MDETR \cite{kamath2021mdetr} & DETR \cite{carion2020end} & 1,3,4 &  & word &  & \checkmark & \checkmark & & & \checkmark & \checkmark & \checkmark \\
  DQ-DETR \cite{} & DETR \cite{carion2020end} & 1,3,4 &  & word & \checkmark & \checkmark & & & & \checkmark & \checkmark & \checkmark \\
  GLIP \cite{li2021grounded} & DyHead \cite{dai2021dynamic} & 1,2 &  & word & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &  & \checkmark & \\
  GLIPv2 \cite{GLIPv2} & DyHead \cite{dai2021dynamic} & 1,2 &  & word & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &  & \checkmark & \\
  OV-DETR \cite{YuhangZang2022OpenVocabularyDW} & Deformable DETR \cite{zhu2020deformable}  & 3,4 & \checkmark & sentence & & \checkmark &&& &&& \\
  OWL-ViT \cite{MatthiasMinderer2022SimpleOO} & - & 2 & \checkmark & sentence & \checkmark & \checkmark & \checkmark && \\
  DetCLIP \cite{LeweiYao2022DetCLIPDV} & ATSS \cite{ATSS} & 2 & \checkmark & sentence & & \checkmark & \checkmark && &&& \\
  OmDet \cite{TianchengZhao2022OmDetLO} & Sparse R-CNN \cite{sun2021sparse} & 3,4 & \checkmark & sentence & \checkmark & \checkmark & \checkmark & \checkmark& \checkmark &&& \\
  Grounding DINO (Ours) & DINO \cite{zhang2022dino} & 1,2,3,4 & & sub-sentence & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
  \bottomrule
\end{tabu}}
\vspace{-0.28cm}
\caption{A comparison of previous open-world object detectors. Our summarization is based on the experiments in their paper, but not the ability to extend their models to other tasks or designs. It is worth noting that some related works may not (only) designed for the open-world object detection initially, like MDETR and GLIPv2, but we list them here for a comprehensive comparison with existing work. 
}
\label{tab:related_work}
\end{center}
\end{table*}

==> tables/related_work2.tex <==
\begin{table*}[h]
\begin{center}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabu}{
l@{\hskip9pt} |  
c@{\hskip9pt} c@{\hskip9pt}  c@{\hskip9pt} |
c@{\hskip9pt} |
c@{\hskip9pt} |
c@{\hskip9pt} c@{\hskip9pt} c@{\hskip9pt} |
c@{\hskip9pt} 
}
 \toprule
 \multirow{2}{*}{Model}  & 
 \multicolumn{3}{c|}{Model Design}  & 
 \multicolumn{1}{c|}{Text Prompt}  & 
 \multicolumn{1}{c|}{Close-Set Settings} &
 \multicolumn{3}{c|}{Open-Set Settings} & 
 \multicolumn{1}{c}{Visual-Grounding Settings}  \\
  & 
  Base Detector & Fusion Phases (Fig. \ref{fig:model_comparison}) & CLIP-dependent & 
  Representation Level & 
  COCO & 
  COCO &  LVIS  & ODinW  &
  RefCOCO/+/g \\
\midrule
  ViLD \cite{XiuyeGu2021OpenvocabularyOD} & Mask R-CNN \cite{he2017mask} & 3,4 & \checkmark & sentence & & \checkmark & &\\
  RegionCLIP \cite{YiwuZhong2022RegionCLIPRL} & Faster RCNN \cite{faster-rcnn} & 4 & \checkmark & sentence & \checkmark & \checkmark & &\\
  FindIt \cite{WeichengKuo2022FindItGL} & Faster RCNN \cite{faster-rcnn} & 3,4 &  & sentence & \checkmark & & & \checkmark \\
  MDETR \cite{kamath2021mdetr} & DETR \cite{carion2020end} & 1,3,4 &  & word &  & \checkmark & \checkmark & \checkmark \\
  DQ-DETR \cite{dqdetr} & DETR \cite{carion2020end} & 1,3,4 &  & word & \checkmark & \checkmark & &\checkmark \\
  GLIP \cite{li2021grounded} & DyHead \cite{dai2021dynamic} & 1,2 &  & word & \checkmark & \checkmark & \checkmark  & \\
  GLIPv2 \cite{GLIPv2} & DyHead \cite{dai2021dynamic} & 1,2 &  & word & \checkmark & \checkmark & \checkmark  & \\
  OV-DETR \cite{YuhangZang2022OpenVocabularyDW} & Deformable DETR \cite{zhu2020deformable}  & 3,4 & \checkmark & sentence & \checkmark & \checkmark && \\
  OWL-ViT \cite{MatthiasMinderer2022SimpleOO} & - & 2 & \checkmark & sentence & \checkmark & \checkmark & \checkmark & \\
  DetCLIP \cite{LeweiYao2022DetCLIPDV} & ATSS \cite{ATSS} & 2 & \checkmark & sentence & & \checkmark & \checkmark & \\
  OmDet \cite{TianchengZhao2022OmDetLO} & Sparse R-CNN \cite{sun2021sparse} & 3,4 & \checkmark & sentence & \checkmark & \checkmark & \checkmark & \\
  Grounding DINO (Ours) & DINO \cite{zhang2022dino} & 1,2,3,4 & & sub-sentence & \checkmark & \checkmark & \checkmark &\checkmark \\
  \bottomrule
\end{tabu}}
\vspace{-0.28cm}
\caption{A comparison of previous open-world object detectors. Our summarization is based on the experiments in their paper, but not the ability to extend their models to other tasks or designs. It is worth noting that some related works may not (only) designed for the open-world object detection initially, like MDETR \cite{kamath2021mdetr} and GLIPv2\cite{GLIPv2}, but we list them here for a comprehensive comparison with existing work. 
}
\label{table:related_work}
\end{center}
\end{table*}

==> tables/related_work3.tex <==
\begin{table*}[htbp]
\begin{center}
\renewcommand{\arraystretch}{1.3}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabu}{
l@{\hskip9pt} |  
c@{\hskip9pt} c@{\hskip9pt}  c@{\hskip9pt} |
c@{\hskip9pt} |
c@{\hskip9pt} |
c@{\hskip9pt} c@{\hskip9pt} c@{\hskip9pt} |
c@{\hskip9pt} 
}
 \toprule
 \multirow{2}{*}{Model}  & 
 \multicolumn{3}{c|}{Model Design}  & 
 \multicolumn{1}{c|}{Text Prompt}  & 
 \multicolumn{1}{c|}{Closed-Set Settings} &
 \multicolumn{3}{c|}{Zero-Shot Transfer} & 
 \multicolumn{1}{c}{Referring Detection}  
 \\
  & 
  Base Detector & Fusion Phases (Fig. \ref{fig:model_comparison}) & use CLIP & 
  Represent. Level (Sec. \ref{sec:sub_sentence}) & 
  COCO & 
  COCO &  LVIS  & ODinW  &
  RefCOCO/+/g \\
\midrule
  ViLD \cite{XiuyeGu2021OpenvocabularyOD} & Mask R-CNN \cite{he2017mask} & - & \checkmark & sentence & \checkmark & partial label & partial label &\\
  RegionCLIP \cite{YiwuZhong2022RegionCLIPRL} & Faster RCNN \cite{faster-rcnn} & - & \checkmark & sentence & \checkmark & partial label & partial label &\\
  FindIt \cite{WeichengKuo2022FindItGL} & Faster RCNN \cite{faster-rcnn} & A &  & sentence & \checkmark & partial label & & & fine-tune \\
  MDETR \cite{kamath2021mdetr} & DETR \cite{carion2020end} & A,C &  & word &  & &  fine-tune & zero-shot & fine-tune \\
  DQ-DETR \cite{dqdetr} & DETR \cite{carion2020end} & A,C &  & word & \checkmark & & zero-shot & & fine-tune \\
  GLIP \cite{li2021grounded} & DyHead \cite{dai2021dynamic} & A &  & word & \checkmark & zero-shot & zero-shot & zero-shot & \\
  GLIPv2 \cite{GLIPv2} & DyHead \cite{dai2021dynamic} & A &  & word & \checkmark & zero-shot & zero-shot & zero-shot & \\
  OV-DETR \cite{YuhangZang2022OpenVocabularyDW} & Deformable DETR \cite{zhu2020deformable}  & B & \checkmark & sentence & \checkmark & partial label & partial label & &  \\
  OWL-ViT \cite{MatthiasMinderer2022SimpleOO} & - & - & \checkmark & sentence & \checkmark & partial label & partial label & zero-shot & \\
  DetCLIP \cite{LeweiYao2022DetCLIPDV} & ATSS \cite{ATSS} & - & \checkmark & sentence & &  & zero-shot & zero-shot & \\
  OmDet \cite{TianchengZhao2022OmDetLO} & Sparse R-CNN \cite{sun2021sparse} & C & \checkmark & sentence & \checkmark &  & & zero-shot & \\
  \midrule
  Grounding DINO (Ours) & DINO \cite{zhang2022dino} & A,B,C & & sub-sentence & \checkmark & zero-shot & zero-shot & zero-shot & zero-shot \\
  \bottomrule
\end{tabu}}
\vspace{-0.4cm}
\caption{A comparison of previous open-set object detectors. Our summarization is based on the experiments in their paper, but not the ability to extend their models to other tasks. It is worth noting that some related works may not (only) be designed for the open-set object detection initially, like MDETR \cite{kamath2021mdetr} and GLIPv2\cite{GLIPv2}, but we list them here for a comprehensive comparison with existing work. 
We use the term ``partial label'' for the settings, where models are trained on partial data (e.g. base categories) and evaluated on other cases. 
% \jianwei{when talking about visual grounding, people also think of phrase grounding like Flickr30k. In this sense, MDETR/GLIP-v1/v2 also report visual grounding performance, but on another dataset?}\shilong{I think so. I modify the name from visual grounding to referring detection.}
\vspace{-0.2cm}
}
\label{table:related_work}
\end{center}
\end{table*}

==> tables/two_table.tex <==
\begin{table}[htbp]
    \centering
  \begin{minipage}{.5\linewidth}
    \centering
        \resizebox{\linewidth}{!}{%
        \begin{tabular}{
        l@{\hskip9pt} |  
        l@{\hskip9pt} |  
        c@{\hskip9pt} c@{\hskip9pt} |
        c@{\hskip9pt}
        % c@{\hskip9pt} |
        % c@{\hskip9pt} c@{\hskip9pt}  c@{\hskip9pt}  
        }
         \toprule
         \multirow{2}{*}{\#ID}  & 
         \multirow{2}{*}{Model}  & 
         \multicolumn{2}{c|}{COCO minival} &
         \multicolumn{1}{c}{LVIS minival} 
         % \multicolumn{1}{c|}{ODinW} & 
         % \multicolumn{3}{c}{Visual-Grounding Settings}  
         \\
          & 
          &
          \small{Zero-Shot} & \small{Fine-Tune} &
          \small{Zero-Shot}
          % Zero-shot &
          % RefCOCO & RefCOCO+ & RefCOCOg 
          \\
        \midrule
          0 & Grounding DINO (Full Model) & 46.7 & 56.9 & 16.1 \\
          \midrule[0.3pt]
          1 & w/o encoder fusion & 45.8 & 56.1  & 13.1 \\
          2 & static query selection & 46.3  & 56.6 &  13.6 \\
          3 & w/o text cross-attention & 46.1 & 56.3 & 14.3 \\
          4 & word-level text prompt & 46.4 & 56.6 & 15.6 \\
          \bottomrule
        \end{tabular}
        }
        \caption{Ablations for our model. All models are trained on the O365 dataset with a Swin Transformer Tiny backbone.}
        \label{table:ablation}
     \end{minipage}%
    \hfill%
    \begin{minipage}{.5\linewidth}
    \centering
        \resizebox{\linewidth}{!}{
        \begin{tabular}{
        l@{\hskip9pt} |  
        % c@{\hskip9pt} |  
        c@{\hskip9pt} c@{\hskip9pt}  |  
        c@{\hskip9pt} |
        c@{\hskip9pt} | 
        c@{\hskip9pt} 
        % c@{\hskip9pt} |
        % c@{\hskip9pt} c@{\hskip9pt}  c@{\hskip9pt}  
        }
         \toprule
         \multirow{2}{*}{Model}  & 
         % \multirow{2}{*}{Backbone}  & 
         % \multirow{2}{*}{Pre-Tran}  & 
         \multicolumn{2}{c|}{Pre-Train Data} &
         \multicolumn{1}{c|}{COCO minival} &
         \multicolumn{1}{c|}{LVIS minival} &
         \multicolumn{1}{c}{ODinW} 
         % \multicolumn{3}{c}{Visual-Grounding Settings}  
         \\
          % & 
          &
          \small{DINO Pre-Train} & \small{Grounded Fine-Tune} &
          Zero-Shot &
          Zero-Shot &
          Zero-Shot
          % Zero-shot &
          % RefCOCO & RefCOCO+ & RefCOCOg 
          \\
          \midrule
          Grounding DINO T  & - & O365 & 46.7 & 16.2 & 14.5 \\
          (from scratch)  & - & O365,GoldG & 48.1 & 25.6 & 20.0  \\
          \midrule
          Grounding DINO T  & O365 & O365          & 46.5 & 17.9 & 13.6 \\
          (from pre-trained DINO)  & O365 & O365,GoldG    & 46.4 & 26.1 & 18.5 \\
          \bottomrule
        \end{tabular}}
        \caption{Transfer pre-trained DINO to Grounding DINO. We freeze shared modules between DINO and Grounding DINO during grounded fine-tuning. All models are trained with a Swin Transformer Tiny backbone. }
        \label{table:dino2grounding}
     \end{minipage}
\end{table}
